Towards Few-Annotation Learning in Computer Vision: Application to Image Classification and Object Detection tasks

In this thesis, we develop theoretical, algorithmic and experimental contributions for Machine Learning with limited labels, and more specifically for the tasks of Image Classification and Object Detection in Computer Vision. In a first contribution, we are interested in bridging the gap between theory and practice for popular Meta-Learning algorithms used in Few-Shot Classification. We make connections to Multi-Task Representation Learning, which benefits from solid theoretical foundations, to verify the best conditions for a more efficient meta-learning. Then, to leverage unlabeled data when training object detectors based on the Transformer architecture, we propose both an unsupervised pretraining and a semi-supervised learning method in two other separate contributions. For pretraining, we improve Contrastive Learning for object detectors by introducing the localization information. Finally, our semi-supervised method is the first tailored to transformer-based detectors.

==> glossary.tex <==
% \newglossaryentry{latex}
% {
%     name=latex,
%     description={Is a markup language specially suited for 
% scientific documents}
% }

\newglossaryentry{scalar}
{
    name=$a$,
    description={A scalar (integer or real)}
}

\newglossaryentry{vector}
{
    name=$\rva$,
    description={A vector}
}

\newglossaryentry{matrix}
{
    name=$\rmA$,
    description={A matrix}
}

\newglossaryentry{set}
{
    name=$\Acal$,
    description={A set}
}

\newglossaryentry{space}
{
    name=$\sA$,
    description={A space}
}

\newglossaryentry{real}
{
    name=$\R$,
    description={The space of real numbers}
}

\newglossaryentry{element_vector}
{
    name=$\rva_i$,
    description={Element $i$ of vector $\rva$, with indexing starting at 1}
}

\newglossaryentry{element_matrix}
{
    name=$\rmA_{(i,j)}$,
    description={Element $i,j$ of matrix $\rmA$}
}

\newglossaryentry{set_int}
{
    name=$[[N]]$,
    description={The set of all integers from 1 to $N$: $[[N]] := \{ 1, \dots, N \}$}
}

\newglossaryentry{param}
{
    name=$\theta$,
    description={Parameters or \emph{weights} of the model}
}

\newglossaryentry{optim}
{
    name=$\theta^*$,
    description={Optimal, or ideal parameters}
}

\newglossaryentry{emp}
{
    name=$\hat{\theta}$,
    description={Empirical parameters}
}

\newglossaryentry{transpose}
{
    name={$\rmA^\top, \rva^\top$},
    description={Transpose of matrix $\rmA$ or vector $\rva$}
}

\newglossaryentry{norm_p}
{
    name=$\|\rvx \|_p$,
    description={$L_p$ norm of $\rvx$}
}

\newglossaryentry{norm_2}
{
    name=$\|\rvx \|$,
    description={$L_2$ norm of $\rvx$}
}

\newglossaryentry{norm_fro}
{
    name=$\|\rmX \|_F$,
    description={Frobenius norm of $\rmX$}
}

\newglossaryentry{prod_scal}
{
    name={$\langle\rvx,\rvy\rangle$},
    description={Scalar product between $\rvx$ and $\rvy$}
}

\newglossaryentry{proba}
{
    name=$P(\rvx)$,
    description={Probability distribution over $\rvx$}
}

\newglossaryentry{distrib}
{
    name=$\rvx \sim P$,
    description={Random variable $\rvx$ has distribution $P$}
}

\newglossaryentry{expectation}
{
    name=$\E_{\rvx \sim P}[f(\rvx)]$,
    description={Expectation of $f(\rvx)$ with $\rvx$ following distribution $P$}
}

\newglossaryentry{gauss}
{
    name={$\gN(\mu,\Sigma)$},
    description={Gaussian distribution with mean $\mu$ and covariance $\Sigma$}
}

\newglossaryentry{indic}
{
    name=$\1_{\text{condition}}$,
    description={function that is 1 if condition is true, 0 otherwise}
}

\newacronym{deep}{DL}{Deep Learning}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{sup}{SL}{Supervised Learning}

\newacronym{semi}{SSL}{Semi-Supervised Learning}
\newacronym{self}{Self-SL}{Self-Supervised Learning}
\newacronym{unsup}{UL}{Unsupervised Learning}

\newacronym{many}{MSL}{Many-Shot Learning}
\newacronym{few}{FSL}{Few-Shot Learning}
\newacronym{fal}{FAL}{Few-Annotation Learning}

\newacronym{amt}{AMT}{Amazon Mechanical Turk}
\newacronym{od}{OD}{Object Detection}
\newacronym{fsc}{FSC}{Few-Shot Classification}
\newacronym{fsod}{FSOD}{Few-Shot Object Detection}
\newacronym{ssod}{SSOD}{Semi-Supervised Object Detection}

\newacronym{mlp}{MLP}{Multi-Layer Perceptron}
\newacronym{cnn}{CNN}{Convolutional Neural Network}

\newacronym{mtr}{MTR}{Multi-Task Representation Learning}
\newacronym{ema}{EMA}{Exponential Moving Average}


\newacronym{coco}{COCO}{Microsoft Common Object in Context dataset}
\newacronym{ilsvrc}{ILSVRC}{ImageNet Large-Scale Visual Recognition Challenge dataset}

\newacronym{pp}{p.p.}{Percentage point}

\newacronym{iou}{IoU}{Intersection over Union, measure the overlap of predicted bounding box to the ground truth}


\newacronym{ap}{AP}{Average Precision metric}
\newacronym{ap50}{$\text{AP}_{50}$}{Average Precision metric calculated at IoU threshold of 0.5}

\newacronym{map}{mAP}{mean Average Precision metric, AP calculated for IoU threshold from 0.5 to 0.95 with step size of 0.05}



==> notations.tex <==
\chapter*{Notation}
\label{notation}

\newlength{\notationgap}
\setlength{\notationgap}{1pc}


% \typeout{START_CHAPTER "notation" \theabspage}

% Sometimes we have to include the following line to get this section
% included in the Table of Contents despite being a chapter*
\addcontentsline{toc}{chapter}{Notation}
This section provides a concise reference describing notation used throughout this
document.

\vspace{\notationgap}
% Need to use minipage to keep title of table on same page as table
\begin{minipage}{\textwidth}
% This is a hack to put a little title over the table
% We cannot use "\section*", etc., they appear in the table of contents.
% tocdepth does not work on this chapter.
\centerline{\bf Numbers and Arrays}
\bgroup
% The \arraystretch definition here increases the space between rows in the table,
% so that \displaystyle math has more vertical space.
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\index{Scalar}
\index{Vector}
\index{Matrix}
\index{Tensor}
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
% NOTE: do not use \R^+, because it is ambiguous whether:
% - It includes 0
% - It includes only real numbers, or also infinity.
% We usually do not include infinity, so we may explicitly write
% [0, \infty) to include 0
% (0, \infty) to not include 0
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\egroup
\index{Scalar}
\index{Vector}
\index{Matrix}
\index{Tensor}
\index{Graph}
\index{Set}
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Linear Algebra Operations}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \mA^\top$ & Transpose of matrix $\mA$ \\
$\displaystyle \mA^+$ & Moore-Penrose pseudoinverse of $\mA$\\
$\displaystyle \mA \odot \mB $ & Element-wise (Hadamard) product of $\mA$ and $\mB$ \\
% Wikipedia uses \circ for element-wise multiplication but this could be confused with function composition
$\displaystyle \mathrm{det}(\mA)$ & Determinant of $\mA$ \\
\end{tabular}
\egroup
\index{Transpose}
\index{Element-wise product|see {Hadamard product}}
\index{Hadamard product}
\index{Determinant}
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\index{Derivative}
\index{Integral}
\index{Jacobian matrix}
\index{Hessian matrix}
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \ra \bot \rb$ & The random variables $\ra$ and $\rb$ are independent\\
$\displaystyle \ra \bot \rb \mid \rc $ & They are conditionally independent given $\rc$\\
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\index{Independence}
\index{Conditional independence}
\index{Variance}
\index{Covariance}
\index{Kullback-Leibler divergence}
\index{Shannon entropy}
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\index{Sigmoid}
\index{Softplus}
\index{Norm}
\end{minipage}

Sometimes we use a function $f$ whose argument is a scalar but apply
it to a vector, matrix, or tensor: $f(\vx)$, $f(\mX)$, or $f(\tX)$.
This denotes the application of $f$ to the
array element-wise. For example, if $\tC = \sigma(\tX)$, then $\etC_{i,j,k} = \sigma(\etX_{i,j,k})$
for all valid values of $i$, $j$ and $k$.


\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Datasets and Distributions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \pdata$ & The data generating distribution\\
$\displaystyle \ptrain$ & The empirical distribution defined by the training set\\
$\displaystyle \sX$ & A set of training examples\\
$\displaystyle \vx^{(i)}$ & The $i$-th example (input) from a dataset\\
$\displaystyle y^{(i)}\text{ or }\vy^{(i)}$ & The target associated with $\vx^{(i)}$ for supervised learning\\
$\displaystyle \mX$ & The $m \times n$ matrix with input example $\vx^{(i)}$ in row $\mX_{i,:}$\\
\end{tabular}
\egroup
\end{minipage}

\clearpage

% \typeout{END_CHAPTER "notation" \theabspage}

